Driving The Last Mile: Characterizing and Understanding Distracted Driving Posts on Social Networks

In 2015, 391,000 people were injured due to distracted driving in the US. One of the major reasons behind distracted driving is the use of cell-phones, accounting for 14% of fatal crashes. Social media applications have enabled users to stay connected, however, the use of such applications while driving could have serious repercussions -- often leading the user to be distracted from the road and ending up in an accident. In the context of impression management, it has been discovered that individuals often take a risk (such as teens smoking cigarettes, indulging in narcotics, and participating in unsafe sex) to improve their social standing. Therefore, viewing the phenomena of posting distracted driving posts under the lens of self-presentation, it can be hypothesized that users often indulge in risk-taking behavior on social media to improve their impression among their peers. In this paper, we first try to understand the severity of such social-media-based distractions by analyzing the content posted on a popular social media site where the user is driving and is also simultaneously creating content. To this end, we build a deep learning classifier to identify publicly posted content on social media that involves the user driving. Furthermore, a framework proposed to understand factors behind voluntary risk-taking activity observes that younger individuals are more willing to perform such activities, and men (as opposed to women) are more inclined to take risks. Grounding our observations in this framework, we test these hypotheses on 173 cities across the world. We conduct spatial and temporal analysis on a city-level and understand how distracted driving content posting behavior changes due to varied demographics. We discover that the factors put forth by the framework are significant in estimating the extent of such behavior.

==> 020related.tex <==
\section{Related Work}
The related work for this paper flows from four different themes. Firstly, we review how impression management is carried out on social media platforms, followed by how risk-taking affects impression management. Then we review the work related to voluntary risk-taking phenomenon on social media. Finally, we conclude our related work by analyzing the video classification methods.

\textbf{Impression Management on Social Media}: Goffman introduced the term ``impression management", which has been widely used to explain the difference between how an individual's behavior presents an idealized version of themselves rather than the more authentic version of them~\cite{goffman1959presentation}. %Goffman metaphorically compared this through the dramaturgical approach, where the actor (individuals) are presenting a different side of themselves while performing (in the presence of other individuals), thus controlling the impressions their audience (peers) have of them. 
Hogan extended this concept to online social media websites, where he presented views on how online social media platforms can be viewed as a stage (connecting back to the dramaturgical approach) as it allows users to control their impressions via status messages, pictures posted, and even chat conversations~\cite{hogan2010presentation}. Self-presentation on social media among teens and their tendency to conform the (multimedia) content that they post with respect to their gender has also been evaluated in prior work~\cite{herring2015teens}. Our work analyzes driving content posted on social media and extends the impression management concept on social media to hypothesize the reasons behind posting such adventurous risk-taking videos.

\textbf{Risk-taking and Impression Management}: Leary et al. analyzed the voluntary risk-taking activities such as avoiding condoms, indulging in narcotics and steroid use, recklessness such as fast driving, and suggested that such risk-taking activities are undertaken to improve the impression of individuals amongst their peers. Finney's experimental study evaluated that members were favorably looked upon when they indulged in behavior that was characterized by higher risks, in addition to characteristics such as success and status ~\cite{finney1978personality}. Characterizing the type of users who are more susceptible to take risks, Doyle et al. discovered that men are more likely to exhibit adventure or reckless behavior than women~\cite{doyle1995male}. In the context of accidents and injuries, adolescents and young adults seem more inclined to participate in activities that would endanger them~\cite{friedman1989health}. %, in order to convey a certain impression and influence other people's perception of them ~\cite{friedman1989health}. 
\hl{Edit Lyng part; Add more references.}
 Lyng introduced the concept of ``edgework" activities, which he defined as those activities that have a threat to one's physical or mental well-being, and provided examples such as skydiving, rock climbing, car racing, etc~\cite{edgework1990lyng}.  %If not readable, remove
 Lyng presented a sociological framework to understand voluntary risk-taking users, rooting the cause of such activities in micro and macro structures of the modern society.
 
\textbf{Risk-taking on social media}: Risk-taking on social media has also been widely studied for different voluntary activities. Lamba et al. covered a much broader case of dangerous selfies, where users posted a perilous self-portrait in dangerous situations such as at an elevation, with a firearm, or inside a water body. They also showed that users often engage in risk-taking activities while taking selfies to post on social media. Of the 232 deaths due to taking dangerous selfies, $12$ could be attributed to driving-related incidents. The authors presented deep-learning models to distinguish between potentially dangerous and non-dangerous selfies~\cite{nanda2018stop}. Similarly, Hart examined young individuals' participation in `intimate edgework` through posting nude self-portraits on Tumblr \cite{hart2017being}. There has been a normative increase in individuals dabbling in risk-taking behavior as a result of various other social media trends such as the Tide Pod Challenge \cite{murphy2018rationality}, the Cinnamon Challenge \cite{grant2013ingesting}, the Salt and Ice Challenge \cite{roussel2016tweens} and the Fire Challenge \cite{ahern2015risky,avery2016fire}. We extend the framework presented by \cite{lamba2017camera} to analyze the risk-taking activities posed in the form of driving videos on social media, a phenomenon that has not been studied before.

\textbf{Video Classification}: 
A major component of our work is to build a classifier which can identify content, where the content creator is driving or is distracted while driving. Baghel et al. proposed a deep-learning classifier to identify distracted driving videos - their underlying classifier was built on the popular VGG-16 model~\cite{baghel2018kiki}. One popular stream of work to classify the content of videos is to apply image-based classifiers on the frames of the video. To this end, He et al. proposed a model that learned the residual functions to out-perform previous competitors in the widely popular ImageNet challenge. Zagoruyko et al. further improved upon the ResNet model and proposed a Wide Residual Network (WRN), which leveraged increased width of the network to improve accuracy. Xie et al. modified the ResNet model by introducing a new hyper-parameter called cardinality to better tune the depth and width of the model. We use some of these models as inspiration and as the basis for our model. Among video classification approaches used for action recognition, \cite{hara2018can}
work on spatiotemporal 3D CNNs stands out and delivers high accuracy on standard action recognition datasets like Kinetics and UCF101. 
% stands out as a seminal work that extensively categorized over 1 million sports videos in almost 500 classes using the concept of a fusion module. \sshashank{recheck this citation, also our baseline now performs better}

% In this work, we address all these discussed themes in the context of distracted driving content posted on online social media. We first try to understand the problem of voluntary risk-taking activity on social media. We analyze its prevalence as a global phenomenon and subsequently undertake regression analysis to determine the demographic covariates that can help best explain the characteristics of users indulging in this risk-taking behavior.

%Psychological studies towards understanding the underlying nature across demographics have been carried out. Several trends and variances across the populace have been noted and highlighted. \citeauthor{hong1978risky}'s psychological study provides evidence in support of culture-value explanation of risk-taking behavior via American and Chinese subjects.  Further insight into the adverse factors and risk brought about by indulging in cell phone use while driving can be attributed to a sense of possession of the cell phone ~\cite{weller2013possession}. In the specific context of distraction-affected driving, it has been found that individuals' inclination to using cell phones while driving correlates with the likelihood of the individuals to engage in accessory risk-taking behavior such as speeding, persistent lane changing, and hard acceleration ~\cite{zhao2013self}. A similar assessment -- texting while driving behavior in high school students identified that offenders are also more accepting of riding with a drunk driver, driving drunk, and less likely of taking safety measures such as wearing a seatbelt ~\cite{olsen2013texting}. The positive relationship between cell phone use and an increase in vehicular crashes has also been studied from an epidemiological point of view~\cite{collet2010phoning}. Furthermore, subject-based studies have outlined that females are 70\% more likely to be found using their mobile devices whilst driving ~\cite{foss2009short}. 

%The dawn of social media websites has introduced a new medium for allowing users to control how people perceive them, generally through the means of posting images and maintaining profiles. Hogan et al. characterized the (What did)

%Research work over the years has focused on the anatomical study of the background leading to human behavior in their social groups. The emergence of the internet has created a new avenue for hazardous self-presentation behaviors to develop and flourish. Further, the dawn of social media websites has introduced a new medium for allowing users to control how people perceive them, generally through the means of posting images, maintaining profiles and web-pages~\cite{hogan2010presentation}. Posting content on their profile allows users to manage their self-presentation to their peers and network and regulate the impression that they make. This has been popularly known as impression management. ~\cite{leary2001impression} have explained how individuals undertake actions in order to manage how they are perceived by others. Popularized by Goffman~\cite{leary1994self}, studying impression management has shown to be crucial in explaining actions related to the mental and physical health of individuals. For instance, people often engage in dangerous risky behaviors such as steroid use, or fast driving in order to enhance their social standing among peers~\cite{goffman1959presentation}. \s{add edgework}

% Related work will flow from the following main directions:

% \subsection{Impression Management on Social Media}
% \begin{itemize}
%     \item Goffman
%     \item Hogan
%     \item More recent studies by PC's/ Senior - PC's in ICWSM. Every study uses this social science theory - we can also look at how people use references for this.
% \end{itemize}

% \subsection{Risk-taking and Impression Management (edgework)}
% \begin{itemize}
%     \item Leary
%     \item Edgework
%     \item Further risk-taking analysis and it's effect on impression management
% \end{itemize}

% \subsection{Risk-taking studies on social media}
% \begin{itemize}
%     \item Our work
%     \item Work on posting nude, disturbing images - Hart
% \end{itemize}

% \subsection{Video Classification approaches}
% \begin{itemize}
%     \item Image Classifiers
%     \item Video Classifiers
%     \item Sampling Techniques / Latest models
% \end{itemize}

==> response.tex <==
\onecolumn

\section{Reviewer response}
We would first like to thank the reviewers for their detailed and constructive feedback of our submission. We have tried our best to incorporate all the comments raised by the reviewers in the previous phase of submissions. Some of the highlights of our changes are as follows:

\begin{itemize}
    \item We increased our dataset size from one week to one month's data and from $137$ cities to $173$ cities. We also collected data at a much more granular level i.e., $1km \times 1km$ instead of $2.5 km \times 2.5km$.
    
    \item We clarify our definition of distracted driving content.
    
    \item To address the deep learning model-related concerns, we did the following - (1) increased the size (almost doubled) of our training and testing set, (2) tested the accuracy of the model on a separate held-out test set thus showing that model is not overfitting. Further, we have shared all the details about the dataset and the model that we think is necessary for reproducibility.                          
    
    \item We restructure our paper in order to explain the implications of our approach, and how it is applicable and can be leveraged by platforms to make the users not partake in such risk-taking behavior.
    %\item We provide a clear definition of distracted driving content and roughly double the size of our training and testing set. We test the robustness of our trained classifier by testing it on a separate held-out test set and establish that the model is not capturing any spatial or  temporal bias. We also report all the technical details related to the classifiers such as the hyperparameters and the distribution of snaps in the training and test sets unlike the last time. 
    %\item We restructure our paper in order to detail out the implications of our insights based on the spatio-temporal patterns and the demographics analysis. We also specify the major threats to validity of our work and enumerate the biases and possible issues in our dataset.
\end{itemize}

% We would like to take this opportunity to express our thanks to the reviewers for the positive feedback and helpful comments for correction or modification. 

% Summarize the reviewers main issues
% \begin{enumerate}
%     \item Dataset size was small
%     \item Robustness of network, lack of data \& technical details missing
%     \item Insights (Interventions) and validity of spatio-temporal analysis
%     \item Demographics - insights?, account for other factors like transportation and all
% \end{enumerate}

\noindent
We address all the reviewers concerns in the next page.

\onecolumn
\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}
% \caption{}
% \hline
ID & Reviewer & Reviewer Comment & Author Response & Sections \\
\midrule
1 & R1 & \begin{minipage}[t]{0.34\columnwidth}
First of all, the study does not exploit a 100\% sure classification of the various posts as "driving content", as only a small percentage of the dataset has been manually labeled, while the rest has been categorized by a machine-learning model (trained on the manually-labeled sample). Even though the performance of such a classifier is shown to be very good (Table 3),  there might still be a high degree of imprecision, especially on the data that have not been manually labeled  (the good performance, in fact, refers to the small sample used for training).
\end{minipage}
& \begin{minipage}[t]{0.34\columnwidth}%
The training and test sets were randomly sampled from the whole dataset. We doubled the amount of our training data thus giving more reliability in the results produced. We further evaluated the accuracy of our model by testing it's performance on held-out instances (5k instances). The classifier was able to detect the correct distracted driving instances even in the held out dataset with reliable precision. Furthermore, the number of snaps that exist in our dataset is in millions and hence doing a manual annotation/analysis to obtain reliable labels is a challenging and time-consuming task that we avoid. By taking these steps, we ensured to a certain extent the reliability of the classifier and justify it's use on the unlabelled dataset. Further to alleviate such claims, we fitted two logistic regression model one on just annotated dataset and other on the inferred dataset (instances labeled by the classifier). We observed that the similar factors (population, gender, number of snaps, developing) were significant. Though their p-value was low, but that could also be because of the small number of instances being used for the regression model.

%\hl{Annotated + Inferred}.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth}Detecting Distracted Driving Content \end{minipage} \\
%=================================================
\midrule
2 & R1 & \begin{minipage}[t]{0.34\columnwidth}
More importantly, even the manually-labeled sample may likely contain wrong labels, as deciding if a certain image or video has been created/posted 
while driving is a very difficult task even for a human being. For instance, what about a photo taken by a passenger (not the driver) of a vehicle? 
This is clearly not "driving content", but, looking at the image/video, a human assessor may easily be misleaded. Similarly, the other way around: what about an image/video that does not contain any "driving evidence", but has been created/posted while driving?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We define distracted driving content as those posts which are made either by people while driving or while being in the passenger seat of a car. We argue that a front or back-seat passenger creating social media content, e.g., a video, could also be a source of distraction for the driver. The definition of distracted driving content does not include snaps that consist of photos taken from outside the vehicle. All annotators were provided with this description of distracted driving content and were given clear instructions on how to use the platform. We obtained a Fleiss-Kappa inter-annotator agreement rate of 0.85, which signifies almost perfect agreement amongst the annotators; thus showing high confidence among the reviewers regarding instances. To further avoid the ambiguity of an annotator's response, we decide on a final label only when at least $2$ out of $3$ annotators agree on the label. The detailed instructions given to the annotators before annotation process and further filtering of their responses helps us alleviate concerns related to the wrongly labeled samples.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Introduction \end{minipage}  \\
\midrule
%=================================================
\end{xtabular*}
% \newpage

\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}
\midrule
3 & R1 & \begin{minipage}[t]{0.34\columnwidth}
Finally, the temporal/spatial analysis may easily rely on wrong data too, as it seems that the time assigned to Snapchat posts corresponds to the time when content has been posted, which can be very different from the time when the content has been created (i.e., the time while the poster was driving, which is the time that matters most). A similar consideration may hold for the spatial analysis, as it is not clear whether the location provided by the Snap Map service refers to the location of the user while posting, or the location of the content of the post. Clearly, the one that matters is the latter, but it can be, again, very different from the former (as, clearly, users may post content while they are in locations other than the one where the post refers to).
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
It is a reasonable assumption to make that a person would upload a snap as soon as they have recorded it. Recording a video earlier and then posting it on Snapchat later is a much more involved process since it requires the user to make at least three more additional steps. Additionally, all snaps uploaded at a different time from when they were recorded appear with a header text "Uploaded from camera roll" which is an unfavorable addition to a snap. While we did not test for exact number of such header appearing in our entire dataset, none of the annotators reported the occurrence of this header text in the approximately 15,000 annotated videos. Furthermore, it can be observed in the heatmaps of Figure 4 that distracted driving snaps are more prevalent on roads, suggesting that most of the distracted driving snaps are uploaded as soon as they are recorded. Another justification for making the assumption that snaps are posted real-time and not later than creation is the design of the application itself. The application opens with the camera, thus increasing the emphasis on creating the content. Once the content is created, it can be saved to the gallery (not posted) or posted instantly. The number of steps hence required to create and post instantly are way lesser than saving and re-posting at a later time. Moreover, we are not sure if Snapchat uses the geo-location of where content was created or where the content was posted to be displayed on SnapMap. 

\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Data Collection \& Dataset \end{minipage}  \\


\midrule
4 & R1 & \begin{minipage}[t]{0.34\columnwidth}
The dataset has a very limited time span (just 6 days), which puts into question the actual generality of the insights provided.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We extend the time-span of our study by collecting data over a period of 1 month from March 16th to April 15th. The dataset now consists of 6.4 million snaps collected from 173 cities all over the world.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Data Collection \& Dataset \end{minipage}  \\
\midrule
5 & R1 & \begin{minipage}[t]{0.34\columnwidth}
The insights of the study are not really impactful. Or, at least, the authors fail in giving convincing motivations how the provided insights may be fruitfully exploited in practice. What's the point of characterizing the spatio-temporal and demographic dynamics of driving content? How these findings can actually be used? In which application scenarios?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We describe in detail the implications and applicability of our approach in the \emph{Discussion} section. The deep learning models can be used to identify distracted driving content posted on social media, and the spatio-temporal analysis can be used to make informed decisions regarding the region and time-specific interventions. Similarly, the analysis of demographics can be used to make targeted individual-level intervention measures and awareness campaigns. Additionally all the key insights and the detection module can be combined effectively to come up with multiple intervention designs.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Discussion \end{minipage}  \\
\midrule

%====================
6 & R2 & \begin{minipage}[t]{0.34\columnwidth}
First, it would be interesting to know how the percentage of non-driving posts in the dataset collected through mechanical turk.  In case of heavily imbalanced datasets, too much data augmentation could lead to overtraining, and this could explain the very high accuracy reported in table 3.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
The percentage of non-driving posts in our training set is 74\% . As the datasets were highly imbalanced, we also compute the precision, recall, and F1 score of the models and report those values as well. The possibility of overtraining/overfitting is unlikely since all our models perform well on both the test and the held-out test sets - both of which were not used to train the model.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\end{xtabular*}


% \onecolumn
\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}
\midrule
7 & R2 & \begin{minipage}[t]{0.34\columnwidth}
Maps in Figure 5 should be more clearly explained: is the central zone of each city richer of driving Snaps because those are the areas where more trafficated roads in the city are?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
In the revised draft, we plot the spatial heatmaps of each city with the boundaries provided by the shapefiles. In case the shapefile of a city isn't available, we use the bounding box instead. We also display the scale of the map on the bottom right, along with the color scale on the left to give an estimate of the number of distracted driving snaps seen. Though we can make some preliminary observations about the concentratedness of some cities' heatmap (e.g., Riyadh's hot spots of high distracted driving content is generally around major highway) by manually looking at all the cities. However, generalizing the insight for all the cities is a challenging task as we do not have access to street level data, and hence we leave it for future work.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Characterizing Temporal \& Spatial Patterns \end{minipage}  \\
\midrule

8 & R2 & \begin{minipage}[t]{0.34\columnwidth}
Examples of potential interventions and design recommendation 
should be given in order to provide an overview of the practical implications
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We detail out the implications of the insights and potential intervention measures in the \textit{Discussion} section.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Discussion \end{minipage}  \\
\midrule

%=================================================
9 & R2 & \begin{minipage}[t]{0.34\columnwidth}
The insights 5-7 infer role of demographics on distracted driving behavior based on geolocation and census data, given that this inference is not direct, 
I would suggest to tune down claims like ""Male are more likely to...""
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We enumerate the limitations of the study in detail in the \textit{Threats To Validity} subsection. We acknowledge the various biases that could possibly creep in while making such inferences and no longer make any absolute claims. We also acknowledge that our analysis might be applicable only for Snapchat and might not generalize well for other platforms and also for other risk-taking behavior. And to this end, we have toned down some of our observations.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Discussion \end{minipage}  \\
\midrule

10 & R4 & \begin{minipage}[t]{0.34\columnwidth}
The section of ‘detecting driving content’ needs to add more details. For instance, in the 5K randomly selected snaps, how many are driving snaps? 
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We have a total of 8634 snaps (videos) in our dataset of which 2242 are positive samples (distracted driving). These videos are further converted into 69,125 images (After frame splitting) that are then used for training the image classifiers. Further details are mentioned in the \textit{Detecting Distracted Driving Content} section
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule
\end{xtabular*}

% \onecolumn
\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}
\midrule
11 & R4 & \begin{minipage}[t]{0.34\columnwidth}
"Based on your finding that the dataset consists of 23.77\% driving snaps (It would be reassuring if the 5K randomly selected snaps also consist of 23\% driving snaps), the annotated snaps probably consist of about 1K driving snaps. Is this enough for transfer learning?
"
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
The number of positive samples (distracted driving videos) in our training set is 2,242, and the total number of negative samples is 6,392. The positive samples thus make up about 25.9\% of all the snaps in the training set. The percentage of distracted driving videos in our entire dataset of 6.4 million samples that were predicted using our classifiers is around 23.56\%. Thus, the annotated snaps also contain a similar number of positive samples as the entire dataset. These number of videos along with augmentations like horizontal flipping and random cropping should be enough for transfer learning. Moreover, for the image-based classifiers, we convert each video into multiple frames, and the training set size for image-classifiers then becomes 69,125. We deal with only two labels, unlike several multi-class classification tasks and transfer learning thus becomes easier. In literature, transfer learning tasks have been known to perform well even for smaller datasets and more number of classes than this~\cite{zeiler2014visualizing}.

\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule
12 & R4 & \begin{minipage}[t]{0.34\columnwidth}
I know you used data augmentation methods to increase the number of driving snaps. But I don’t think this can solve the imbalance issue, considering there are only about 1K positive samples.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
In the revised version, we increase the size of our annotated dataset, and after augmentation the class imbalance was reduced notably. This made transfer learning a straightforward process.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule
13 & R4 & \begin{minipage}[t]{0.34\columnwidth}
Besides, how many images did you use to retrain the deep learning models in both image-based methods and video-based methods?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We have a total of 8,634 snaps (videos) in our dataset of which 2,242 are positive samples (distracted driving). These videos are further converted into 69,125 images (after frame splitting) that are then used for training the image classifiers. Additionally, we utilise data augmentation (horizontal flipping, zooming, and rotating for image classifiers and random cropping for video classifiers) during both training and testing phases.

\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage} \\
\midrule
14 & R4 & \begin{minipage}[t]{0.34\columnwidth}
Before data augmentation, what is the proportion of driving snaps and non-driving snaps? This proportion can be used as a baseline to compare the accuracy of your algorithms.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
The ratio of positive samples (distracted driving) and negative samples (non-distracted driving) before data augmentation is 25.9\% and 74.1\% respectively. A baseline classifier that predicts the majority class all the time will arguably have an accuracy of around 74\%. All the proposed models comfortably better this baseline accuracy.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule
15 & R4 & \begin{minipage}[t]{0.34\columnwidth}
About the tiles and localized region: It has been mentioned that the content on Snap Map only has the location information of localized regions without an exact location. How large are these localized regions compared to 2.4km * 2.4km tiles? How did you convert from localized regions into tiles? Did you use the centroid of each localized regions? Also in Juhasz and Hochmair’s paper, they mentioned “Data collection utilized Web Map Tile Service (WMTS) tiles on the 14th zoom level. On this level, a tile covers approximately an area of 2.4 km x 2.4 km.”, which is much easier to understand the concepts of tiles. 
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We employ a method similar to Juhasz and Hochmair's paper and use a tile size of 1km x 1km instead of the 2.4km used by them. We also ensure that all the tiles for a given city lie within the boundaries of the city whenever a shapefile of the city is available on an official source like Open Street Maps. To convert the localized regions into tiles, we divide the city into grids of size 1km x 1km based on its bounding box or shapefile and remove all the tiles that lie outside the city's boundary. 
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Data Collection \& Dataset \end{minipage}  \\
\end{xtabular*}
% \midrule
% \hline

\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}
% \hline
\midrule
16 & R4 & \begin{minipage}[t]{0.34\columnwidth}
I cannot tell the difference between Figure 3 and Figure 4(a). Aren’t they the same except with different visualization types?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
Both these plots depict the same result, albeit in a different manner. Thus, the radial plots have been removed from the paper as they do not convey anything significantly different. 
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Characterizing Spatial \& Temporal Patterns \end{minipage}  \\

\midrule
17 & R4 & \begin{minipage}[t]{0.34\columnwidth}
If a passenger who sits next to the driver created a driving snap, is this driving snap or not based on your algorithm?
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We define distracted driving content as all the snaps (videos) which are made while people are driving or are in the passenger seat. Arguably a front-seat passenger creating social media content, e.g., a video, could also be a source of distraction for the driver.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Characterizing Spatial \& Temporal Patterns \end{minipage}  \\
\midrule


% \onecolumn
18 & R4 & \begin{minipage}[t]{0.34\columnwidth}
In the section of ‘Effect of Variables’, you can add population density as a new factor. This would make more sense since you explain the coefficient of population in terms of traffic and congestion.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We do not consider population density as a variable for our regression analysis as the area of the city that we consider in our data collection (calculated through either shapefiles or bounding boxes) and the actual area of the city (according to official sources) might be different. For example, few cities do not provide any shape file data and we collect the data from the whole bounding box of the city which does not accurately reflect the actual are of the city.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Characterizing Users \end{minipage}  \\
\midrule
%+===============================================
19 & R5 & \begin{minipage}[t]{0.34\columnwidth}
For a future revision of this paper, I would encourage the authors to collect more data. R1 points out that the dataset was collected over only 6 days -- a much too small time span to be able to eliminate concerns about idiosyncratic effects due to increased or decreased driving activity -- for instance, due to holidays or sporting events.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
For the revision, we collected a month's data (31 days) from March 16th - April 15th. Thus, concerns of idiosyncrasies like increased/decreased driving activity due to holidays or sports are removed.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Data Collection \& Dataset \end{minipage}  \\
\midrule
%==================================================
20 & R5 & \begin{minipage}[t]{0.34\columnwidth}
Additionally, R4 points out that more positive examples are needed, as the current number of positive examples is insufficient even for transfer learning.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
Solved using more training data, augmentation as mentioned in response ID number 11. We also test the robustness of all the models on a separate held-out test set to verify that our models generalize well over the entire dataset.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule
21 & R5 & \begin{minipage}[t]{0.34\columnwidth}
The authors could test whether classifier errors are associated with their predictor variables (perhaps using a Chi-square test for discrete predictors, or a two-sample t-test for continuous ones). Another robustness check would involve analyzing the labeled data as well as the classified data: if both datasets are suggestive of the same conclusion (at least at a high level), this would further strengthen the analysis.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We performed a robustness check where we trained the logistic regression model on only the annotated dataset and compared its performance with the overall inferred dataset. We discovered that both the models were performing similarly i.e. the same factors were significant. However, for annotated dataset the significance level was low but we hypothesize that it could have been due to less number of instances for certain cities. 
%We establish that our classifiers are not capturing any specific geographic or temporal bias. To this end, we train a random forest classifier based on geographic features (latitude, longitude) and temporal features (local time of posting) and measured the performance of said classifier. We find that these models
%can barely outperform a baseline classifier that predicts distracted driving content labels 23.56\% of the time. We report these results in Table 5. Hence, we prove that classifier errors aren't associated with any spatial or temporal features. 
%The percentage of the distracted driving snaps in the labelled data is 25.9\% as compared to the 23.56\% in the entire dataset as predicted by our proposed model. This suggests that the there were no inherent biases in the training data. 
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Detecting Distracted Driving Content \end{minipage}  \\
\midrule


\end{xtabular*}
%================
\begin{xtabular*}{\textwidth}{p{0.2cm}p{1.4cm}lll}

\midrule
22 & R5 & \begin{minipage}[t]{0.34\columnwidth}
Another issue raised by both R1 and R3 concerns the construct validity of the labels. "Content created in a moving car," as R1 points out, is not the same as "content created by the driver of a moving car." Given the inherently risky nature of taking photos while driving, it is quite likely that the majority of content identified by the authors is of the former, rather than latter type. Even identifying content created in a moving car would be a worthwhile goal, since truly dangerous content of the "selfie-while-driving" type is likely to be found in this set.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We define distracted driving content clearly in this revision of the submission. The same definition was provided to the annotators at the time of labelling. Distracted driving content is defined as 
those posts which are made either by people while driving or while being in the passenger seat of a car. We thus consider all posts made by a passenger in the car as distracted driving content. By the same definition, we consider all types of content generated in a car as distracted driving content. However, the definition of distracted driving content does not include snaps that consist of photos taken from outside the vehicle. 
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Introduction \end{minipage}  \\
\midrule
23 & R5 & \begin{minipage}[t]{0.34\columnwidth}
Another issue for the authors to consider is the competition between economic and social-psychological explanations. I applaud a paper that builds on Goffman's micro-sociological theory, but I have to point out how self-presentation concerns are not the only potential explanation. As Table 5 shows, driving content seems to occur more in developing world cities, which likely also lack public transportation, leading to more people driving, *especially* to more of Snapchat users driving -- Snapachat users likely being a self-selected younger, wealthier and higher-educated demographic. 
Without a way to normalize for prevalence of driving, analyzing the spatial distribution of driving snap content becomes a lot more tenuous.
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
Yes, we agree that self-presentation concerns are not the only potential explanations. Hence, for the revised draft, we dig up more interesting sociological framework i.e., \emph{edgework}, and test the possible factors listed there to see if they are able to explain the phenomenon. We additionally agree with the reviewer's point about normalizing the prevalence of driving. However, lack of availability of driving data for all cities we analyzed, we instead introduced multiple control variables that allow us to be able to analyze the number of distracted driving snaps reasonably well. For example, the economic status of the city acts as a proxy for various factors such as internet penetration, social media usage, and use of public transport, etc. and similarly the number of total snaps control for the usage of the Snapchat by the population of the city.
%We use the economic status of a city as one of the variables in our study, which acts as a proxy for various other additional variables for which data is less readily available such as smartphone penetration, social media usage, availability of public transportation facilities, and prevalence of driving. Besides this, we also account for certain other control variables such as the total number of snaps posted in the city and population of the city as a natural control for the popularity of Snapchat in the city. 
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Discussion \end{minipage}  \\
\midrule
% \onecolumn
24 & R5 & \begin{minipage}[t]{0.34\columnwidth}
In my view, building a robust dataset that contains real images of "Snapchatting-while-driving" behavior is a hard enough task, and the authors do not necessarily have to dig deep into the patterns in their data. However, as R1 points out, if the authors do decide to provide insights w/r to spatio-temporal patterns, the rationale for doing so requires explanation. Before trying to analyze these patterns, perhaps a more fundamental concern would be ensuring the validity of the classifier, and delving deeper into its implementation. All reviewers point out the fact that important technical details are missing from the paper. The authors may consider allocating more space for such details, rather than for insights based on the classifier (for which a future paper is always an option!).
\end{minipage} & 
\begin{minipage}[t]{0.34\columnwidth}
We have verified and validated the robustness of the proposed approach by testing on an held-out test set. We also detail out the exact data augmentation techniques and hyper-parameters used for training. We also report all the technical details of the classifiers like the hyperparameters and the distribution of snaps in the training and test sets. Our proposed approach can detect distracted driving content with very high accuracy. However, in order to completely tackle the problem of distracted driving posts on social media, it is necessary to understand the economic and other social factors behind such a phenomenon. The remaining sections on spatio-temporal analysis and characterizing users focus on the same and can be used by platform designers and policymakers to make informed measures. We discuss the implications of our insights in detail in the \textit{Discussion} section. Furthermore, we will release our classifier code and the dataset we have collected to ensure that all our analysis is reproducible.
\end{minipage} & \begin{minipage}[t]{0.11\columnwidth} Discussion \end{minipage}  \\
\bottomrule
% \hline
% 26 & R1 & \begin{minipage}[t]{0.34\columnwidth}

% \end{minipage} & 
% \begin{minipage}[t]{0.34\columnwidth}

% \end{minipage} & column5  \\
% \hline
\end{xtabular*}
% \twocolumn
